Fair Hierarchical Clustering

As machine learning has become more prevalent, researchers have begun to recognize the necessity of ensuring machine learning systems are fair. Recently, there has been an interest in defining a notion of fairness that mitigates over-representation in traditional clustering. In this paper we extend this notion to hierarchical clustering, where the goal is to recursively partition the data to optimize a specific objective. For various natural objectives, we obtain simple, efficient algorithms to find a provably good fair hierarchical clustering. Empirically, we show that our algorithms can find a fair hierarchical clustering, with only a negligible loss in the objective.

==> cost_algorithm_2.tex <==
\section{Pseudocode for the cost objective}

\begin{algorithm}[tb]
   \caption{Fair Hierarchical Clustering for Cost}
   \label{alg:cost}
\begin{algorithmic}
   \STATE {\bfseries Input:} graph $G $, edge weight function $w:E\to\mathbb{R}$, color function $c:V\to\{\text{RED,BLUE}\}$, parameters $t$ and $\ell$
   \STATE $T = \textsc{UnfairHC}(G,w)$
   \COMMENT{Blackbox unfair clustering, Step (A)}
   \STATE Run Algorithms 3-8 \COMMENT{Steps (B)-(G)}
   %\STATE $\mathcal{C} = \textsc{GetMaximalClustering}(t,T)$ \COMMENT{Step (B)}
   %\STATE $\mathcal{C}_0 = \textsc{CombineClusters}(t,\mathcal{C})$\COMMENT{Step (C)}
   %\STATE $ex, exc = \textsc{FindExcess}(G, c, \mathcal{C}_0)$\COMMENT{Step (D)}
   %\STATE $H_M, root = \textsc{ConstructClustGraph}(G, c, \ell, \mathcal{C}_0,ex, exc)$\COMMENT{Step (E)}
   %\STATE $freeRVerts, freeBVerts = \textsc{FixUnmatchedVerts}(H_M, root, c, \ell, \mathcal{C}_0, ex, exc)$\COMMENT{Step (F)}
   %\STATE $\mathcal{C}' = \textsc{ConstructClust}(\mathcal{C}_0, H_M, freeRVerts, freeBVerts)$\COMMENT{Step (G)}
   \STATE Return $\mathcal{C}'$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
   \caption{Get Maximal Clustering, Step (B)}
   \label{alg:stepb}
\begin{algorithmic}
   %\STATE {\bfseries Input:} $t$ a threshold, $T$ a clustering tree of $G$ (vertices are clusters)
   \STATE Let $\mathcal{C} = \emptyset$
   \FOR{$C$ with $|C|\leq t$ in a \textsf{BFS} of $T$}
   \STATE Put $C$ in $\mathcal{C}$
   \STATE Do not proceed to $C$'s children
   \ENDFOR
    \STATE Return $\mathcal{C}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
   \caption{Combine Clusters, Step (C)}
   \label{alg:stepc}
\begin{algorithmic}
   %\STATE {\bfseries Input:} $t$ a threshold, $\mathcal{C}$ a clustering
   \STATE $\mathcal{C}_0, nextC = \emptyset$
   \FOR{$C$ {\bfseries in} $\mathcal{C}$}
   \STATE $nextC \leftarrow nextC\cup C$
   \IF{$|nextC| \geq t$}
   \STATE Add $nextC$ to $\mathcal{C}_0$
   \STATE $nextC = \emptyset$
   \ENDIF
   \ENDFOR
   \STATE If applicable, merge the remaining $nextC$ into some element in $\mathcal{C}_0$
   \STATE Return $\mathcal{C}_0$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
   \caption{Find Excess, Step (D)}
   \label{alg:stepd}
\begin{algorithmic}
   %\STATE {\bfseries Input:} graph $G$, color function $c:V\to\{\text{RED,BLUE}\}$, clustering $\mathcal{C}_0$ of $G$
   \STATE Init excess function $ex:\mathcal{C}_0\to\mathbb{N}$
   \STATE Init excess color function $exc:\mathcal{C}_0 \to\{\text{RED,BLUE}\}$
   \FOR{$C$ {\bfseries in} $\mathcal{C}_0$}
   \STATE Let $exc(C)$ be the majority color in $C$
   \STATE Let $ex(C)$ be the difference between majority and minority colors in $C$
   \ENDFOR
   \STATE Return $ex, exc$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
   \caption{Construct Clustering Graph, Step (E)}
   \label{alg:stepe}
\begin{algorithmic}
   %\STATE {\bfseries Input:} graph $G$, color function $c:V\to\{\text{RED,BLUE}\}$, parameter $\ell$, clustering $\mathcal{C}_0$, excess functions $ex:\mathcal{C}_0\to\mathbb{N}$ and $exc:\mathcal{C}_0\to\{\text{RED,BLUE}\}$
   \STATE Init clustering graph $H_M= (V_M=\mathcal{C}_0,E_M)$, let $K_H$ be its components throughout the algorithm
   %\STATE Init $V_M = \{C_i\in \mathcal{C}_0: ex(C_i) \geq \ell\}$
   %\STATE Init function $root:K_H\to V_M$ where if $k_{C_i} = \{C_i\}$ for $C_i\in V_M$, $root(k_{C_i})= C_i$
   \STATE Let $C_i\in V_M$ be some starting point
   %\STATE Let $compSize = 1$
   \WHILE{$\exists$ an unvisited $C_j\in V_M$ such that $exc(C_j)\neq exc(C_i)$} 
   \STATE Add $(C_i,C_j)$ to $E_M$
   %\STATE $compSize += 1$
   \STATE Swap labels $C_i$ and $C_j$ if $ex(C_j) > ex(C_i)$
   \STATE Set $ex(C_i) \leftarrow ex(C_i) - ex(C_j)$
   \IF{$ex(C_i) < \ell$ or $|k_{C_i}| >= \ell$}
   \STATE Reassign starting point $C_i$ to an unvisited vertex in $V_M$
   %\STATE Let $compSize = 1$
   \ENDIF
   \ENDWHILE
   \STATE Return $H_M, root$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
   \caption{Fix Unmatched Vertices, Step (F)}
   \label{alg:stepf}
\begin{algorithmic}
   %\STATE {\bfseries Input:} graph $H_M$ with components $K_H$, root function $root:K_H\to V_M$, color function $c:V\to\{\text{RED,BLUE}\}$, parameters $t$ and $\ell$, clustering $\mathcal{C}_0$, excess functions $ex:\mathcal{C}_0\to\mathbb{N}$ and $exc:\mathcal{C}_0\to\{\text{RED,BLUE}\}$
   \STATE Init $freeVerts: \mathcal{C}_0\times\{\text{RED,BLUE}\}\to \mathbb{N}$
   \STATE Let $nSteps = 108t^2/\ell^3$ \COMMENT{derived in Appendix}
   \FOR{$C\in\mathcal{C}_0\setminus V_M$}
   \STATE Set $freeVerts(C,\text{RED}), freeVerts(C,\text{BLUE})  = m^2/\ell^2$
   \ENDFOR
   \FOR{$i$ {\bfseries from} $1$ {\bfseries to} $nSteps$}
   \FOR{Component $k$ {\bfseries in} $K_H$}
   \FOR{$p$ {\bfseries in} a \textsf{BFS} of $k$}
   \STATE Let $ch$ be some child of $p$
   \STATE Add $\ell$ to $freeVerts(p, exc(p))$, remove $\ell$ from $ex(p)$
   \STATE Add $\ell$ to $freeVerts(ch,exc(ch))$, remove $\ell$ from $ex(ch)$
   \IF{Less than $\ell$ matches between $p$ and $ch$ remain}
   \STATE Remove $(p,ch)$ from $E_M$, creating new component $k'\in K_H$
   \ENDIF
   \ENDFOR
   \ENDFOR
   \ENDFOR
   \STATE Return $freeVerts$
\end{algorithmic}
\end{algorithm}

\iffalse
\begin{algorithm}[tb]
   \caption{Break Components}
   \label{alg:stepff}
\begin{algorithmic}
   %\STATE {\bfseries Input:} component tree $K\in K_H$, vertex $p\in V(K)$, graph $H_M$ with components $K_H$, root function $root:K_H\to V(H_M)$, color function $c:V\to\{\text{RED,BLUE}\}$, parameter $\ell$, clustering $\mathcal{C}_0$, excess functions $ex:\mathcal{C}_0\to\mathbb{N}$ and $exc:\mathcal{C}_0\to\{\text{RED,BLUE}\}$
   \STATE Find some $c$ child of $p$
   \IF{$exc(p) == \text{RED}$}
   \STATE $freeRVerts(p) += \ell$
   \STATE $freeBVerts(c) += \ell$
   \ELSE 
   \STATE $freeRVerts(c) += \ell$
   \STATE $freeBVerts(p) += \ell$
   \ENDIF
   \STATE $ex(p) -= \ell$
   \STATE $ex(p) -= \ell$
   \IF{Less than $\ell$ matches between $p$ and $c$ remain}
   \STATE Remove $(p,c)$ from $E(H_M)$
   \STATE For new component $K'$, set $root(K') = c$
   \ENDIF
\end{algorithmic}
\end{algorithm}
\fi


\begin{algorithm}[tb]
   \caption{Construct Clustering, Step (G)}
   \label{alg:stepg}
\begin{algorithmic}
   %\STATE {\bfseries Input:} graph $G$, graph $H_M$, color function $c:V\to\{\text{RED,BLUE}\}$, parameter $\ell$, clustering $\mathcal{C}_0$, excess functions $ex:\mathcal{C}_0\to\mathbb{N}$ and $exc:\mathcal{C}_0\to\{\text{RED,BLUE}\}$
   \STATE Let $\mathcal{C}'=\emptyset$
   \STATE Let $removedVerts = \emptyset$
   \FOR{$C$ in $\mathcal{C}_0$}
   \FOR{$color$ {\bfseries in} $\{\text{RED, BLUE}\}$}
   \STATE Let $f = freeVerts(C, color)$
   \STATE Let $C_f = \{v\in C:c(v)=color\}$
   \STATE Create the transformed graph $L$ \COMMENT{Described in the proof of Lemma~\ref{lem:weightloss}}
   \STATE $C' = \textsc{MinWeightBisection}(L)$ \COMMENT{Blackbox, returns isolated $C_f$ vertices}
   \STATE $C = C\setminus C'$
   \STATE $removedVerts = removedVerts \cup C'$
   \STATE $ex(C) -= |C'|$
   \ENDFOR
   \ENDFOR
   \FOR{$C\in \mathcal{C}_0$}
   \STATE Let $S\subset removedVerts$ such that $|S| = ex(C)$ with no vertices of color $exc(C)$
   \STATE $C = C\cup S$
   \STATE $removedVerts = removedVerts \setminus S$
   \STATE Add $C$ to $\mathcal{C}'$
   \ENDFOR
   \STATE Return $\mathcal{C}'$
\end{algorithmic}
\end{algorithm}
